Absence of submultiplicative norms for Wick-ordered Operator Products

In this paper, a key problem of the rigorous formulation of the renormalization group as a continuous flow is identified. Some essential features of the operator-theoretic renormalization group are recalled, and a family of norms associated to different Banach spaces of Hamiltonians is introduced. From this, three different properties, which should be satisfied by an adequate norm, are derived, e.g., a submultiplicativity with respect to Wick-ordering. A proof is given that none of the norms introduced in this paper satisfy all of these conditions.

==> Introduction.tex <==
This paper is about norms for interaction operators on the bosonic Fockspace $\mathcal{F}_b(L^2(\mathbb{R}^d))$, arising from spectral problems in Quantum Field Theory. It is based on \cite{sfb}, \cite{haslerherbst}. In the context of Renormalization-Group methods it is usual to represent an interaction $W \in \mathcal{B}(\mathcal{F}_b(L^2(\mathbb{R}^d)))$ by its components $(W_{m,n})_{m+n \geq 1} \subseteq \mathcal{B}(\mathcal{F}_b(L^2(\mathbb{R}^d)))$ describing interactions where $n$ particles get destroyed and $m$ particles get created, such that $W = \sum_{m+n\geq 1} W_{m,n}$. We characterise these operators $W_{m,n}$ by their integral kernels and define a most general family of norms for these kernels. The main result of this paper is, that there are no norms for the interaction operator kernels satisfying a submultiplicity in terms of estimating the norm of the normal-ordered product of two interactions by their individual norms.\\
To be more precise, we define the field energy operator
\begin{equation}
    H_{ph} = \int_{\mathbb{R}^d}\limits \dd^dk a^\ast(k) \vert k\vert a(k)
\end{equation}
for mass-less, scalar bosons in $d \in \mathbb{N}$ dimensions on the bosonic Fockspace $\mathcal{F}_b(L^2(\mathbb{R}^d))$. Here $(a^\ast(k), a(k))$ mean the pointwise bosonic creation- and annihilation-operators, defined as operator-valued distributions, such that
\begin{equation}
    [a(k), a(k^\prime)] = 0 = [a^\ast(k), a^\ast(k^\prime)] \quad, \quad [a(k), a^\ast(k^\prime)] = \delta^d(k-k^\prime).
\end{equation}
Since our results have nothing to do with UV-divergences, we prove them for the case of small field energies restricting the analysis to the reduced Hilbert-space $\mathcal{H}_{red}\coloneqq P_{red} \mathcal{F}_b(L^2(\mathbb{R}^d))$, where $P_{red} = \mathbf{1}[H_{ph} < 1]$ means the projection onto the field energies less than one. The creation and annihilation of $m$ and $n$ particles gets described by the interaction operator
\begin{equation}
    W_{m,n}[w_{m,n}] \coloneqq P_{red} \int_{B_1^{m+n}} \limits \frac{\dd k_1^{m} \dd\Tilde{k}_1^n}{\vert k_1^m\vert^{1/2}\vert \Tilde{k}_1^n\vert^{1/2}} a^\ast(k_1^m) w_{m,n}[H_{ph}; k_1^m; \Tilde{k}_1^n] a(\Tilde{k}_1^n) P_{red} \label{eq: WmnDef},
\end{equation}
where a priori $w_{m,n}: [0,1]\times B_1^{m+n} \mapsto \mathbb{C}$ is a measurable function, which is continuously differentiable in the first argument for almost every $(k_1^m; \Tilde{k}_1^n) \in B_1^{m+n}$. Here, we introduced the notation
\begin{align}
    k_1^m \coloneqq (k_1, ..., k_m) \in \mathbb{R}^{dm} \quad, \quad \Tilde{k}_1^n \coloneqq (\Tilde{k}_1, ..., \Tilde{k}_n) \in \mathbb{R}^{dn},\\
    \dd k_1^m \coloneqq \prod_{i=1}^m \dd^dk_i \quad, \quad a^\ast(k_1^m)\coloneqq \prod_{i=1}^m a^\ast(k_i)\\
    \vert k_1^m\vert \coloneqq \prod_{i=1}^m \vert k_i\vert \quad, \quad \Sigma[k_1^m] \coloneqq \sum_{i=1}^m \vert k_i\vert\\
    B_1^m \coloneqq B_1 \times B_1\times... \times B_1 \quad, \quad B_1 \coloneqq \{k \in \mathbb{R}^d \vert \vert k\vert \leq 1 \}.
\end{align}
Next, we define a family of norms $\Vert \cdot \Vert_{\lambda, p}^\#$ for the functions $w_{m,n}$ in order to have a Banach-space of functions $\mathcal{W}^\#_{m, n}$. Let $\lambda \in \mathbb{R}$ and $p \geq 1$, then we set
\begin{align}
    \Vert w_{m,n}\Vert^\#_{\lambda, p} \coloneqq \Vert w_{m,n}\Vert_{\lambda, p} + \Vert \partial_r w_{m,n} \Vert_{\lambda, p},
\end{align}
where
\begin{equation}
    \Vert w_{m,n}\Vert_{\lambda, p} \coloneqq \left(\int_{B_1^{m+n}}\limits \frac{\dd k_1^m \dd \Tilde{k}_1^n}{\vert k_1^m\vert^{\lambda}\vert\Tilde{k}_1^n\vert^{\lambda}} \sup_{r \in [0,1]} \left\vert w_{m,n}[r; k_1^m; \Tilde{k}_1^n] \right\vert^p \right)^{1/p}
\end{equation}
for $p < \infty$ and
\begin{equation}
    \Vert w_{m,n}\Vert_{\lambda, \infty} \coloneqq \underset{(k_1^m, \Tilde{k}_1^n)\in B_1^{m+n}}{\text{ess sup}} \frac{\sup_{r\in [0,1]}\vert w_{m,n}[r;k_1^{m}; \Tilde{k}_1^{n}]\vert}{\vert k_1^{m}\vert^\lambda \vert \Tilde{k}_1^{n}\vert^\lambda}
\end{equation}
for $p = \infty$. In \cite{sfb} it was shown, that for $p =2$ and $\lambda > 3$ \eqref{eq: WmnDef} indeed defines a bounded operator, if $w_{m,n} \in \mathcal{W}^\#_{m,n}$. In this case one has
\begin{equation}
    \Vert W_{m,n}[w_{m,n}] \Vert_{op} \leq \frac{\Vert w_{m,n}\Vert_{\lambda, 2}}{\sqrt{m^m n^n}}.
\end{equation}
In the $m=0=n$-case, we set
\begin{align}
    \Vert w_{0,0}\Vert^\#_{\lambda, p} \coloneqq& \Vert w_{0,0}\Vert_{\lambda, p} + \Vert \partial_r w_{0,0}\Vert_{\lambda, p}\\
    \Vert w_{0,0}\Vert_{\lambda, p} \coloneqq& \sup_{r \in [0,1]} \vert w_{0,0}[r]\vert
\end{align}
and
\begin{equation}
    W_{0,0}[w_{0,0}] = w_{0,0}[H_{ph}].
\end{equation}
Introducing a weight function $D: \mathbb{N}\cup \{0\} \mapsto \mathbb{R}_{>0}$, we define
\begin{equation}
    \mathcal{W}^D_{\lambda, p} \coloneqq \bigoplus_{m,n \geq 0} \mathcal{W}^\#_{m, n}
\end{equation}
to be the Banach-space of sequences $\underline{w} = (w_{m,n})_{m,n \geq 0} \in \mathcal{W}^D_{\lambda, p}$ for which
\begin{equation}
    \Vert \underline{w}\Vert^D_{\lambda, p} \coloneqq \sum_{m,n\geq 0} D(m) D(n) \Vert w_{m,n}\Vert^\#_{\lambda,p} < \infty \label{eq: DlambdapNormDef}.
\end{equation}
Intuitively, we would like to choose $\lambda, p$ and $D$ such that $\Vert \cdot \Vert^D_{\lambda, p}$ satisfies the following three conditions:

\begin{hypo}\label{hy: norms}
Let $\Vert\cdot\Vert^D_{\lambda, p}: \mathcal{W}^D_{\lambda, p}\mapsto \mathbb{R}_{\geq 0}$ be defined by \eqref{eq: DlambdapNormDef}.
\begin{enumerate}
    \item $\Vert \cdot \Vert_{\lambda, p}^D$ controls the operator norm, such that
    \begin{equation}
        \Vert W[\underline{w}] \Vert_{op} \leq C_{D, \lambda, p} \Vert \underline{w}\Vert^D_{\lambda, p} \label{eq: OpNormDominanz}
    \end{equation}
    for some finite constant $C_{D, \lambda, p}$, where
    \begin{equation}
        W[\underline{w}] = w_{0,0}[H_{ph}] + \sum_{m+n \geq 1} W_{m,n}[w_{m,n}].
    \end{equation}
    \item There is a well-defined product $\ast: \mathcal{W}^D_{\lambda, p} \times \mathcal{W}^D_{\lambda, p} \mapsto \mathcal{W}^D_{\lambda, p}$ such that
    \begin{equation}
        W[\underline{w}_1] W[\underline{w}_2] = W[\underline{w}_1\ast \underline{w}_2]. \label{eq: Algebrenhomomorphismus}
    \end{equation}
    \item $\Vert \cdot\Vert^D_{\lambda, p}$ is a submultiplicative norm w.r.t. the product $\ast$ from \eqref{eq: Algebrenhomomorphismus}, meaning that
    \begin{equation}
        \Vert (\underline{w}_1 \ast \underline{w}_2) \Vert^D_{\lambda, p} \leq C^\prime_{D, \lambda, p} \Vert \underline{w}_1\Vert^D_{\lambda, p} \cdot \Vert \underline{w}_2\Vert^D_{\lambda, p} \label{eq: QuasiSubmultipl}
    \end{equation}
    for a second finite constant $C^\prime_{D, \lambda, p}$.
\end{enumerate}
\end{hypo}

\noindent The main result of this work is, that none of the proposed norms satisfy Hypothesis \ref{hy: norms}. To be more precise, the main result is summarised in the following Theorem.

\begin{theorem}
   Let $\lambda \in \mathbb{R}, p \geq 1$ and $D: \mathbb{N}_0 \mapsto \mathbb{R}_{>0}$ satisfy either
    \begin{itemize}
        \item[(a)] $\liminf_{M \to \infty} \tfrac{D(M)}{D(M+1)} > 0$ or
        \item[(b)] $ \lim_{M \to \infty}\tfrac{D(M)}{D(M+1)} = 0$. 
    \end{itemize}
    Then $\Vert \cdot\Vert^D_{\lambda, p}$, defined as before, does not fulfill Hypothesis \ref{hy: norms}.
\end{theorem}


\noindent The proof of this theorem is done in several steps:
\begin{itemize}
    \item For $p \in [1, 2)$ there are $w_{m,n} \in \mathcal{W}^\#_{m,n}, \Vert w_{m,n}\Vert^\#_{\lambda, p} < \infty$ such that $W_{m,n}[w_{m,n}] \notin \mathcal{B}(\mathcal{H}_{red})$ independently of $D$ (Section \ref{sec: Necconditions}). Roughly speaking, this is a consequence of the fact that $\mathcal{H}_{red}$ is a space of square-integrable functions and the inclusion $L^2(B_1^{m+n}) \subsetneq L^p(B_1^{m+n})$ for $2>p$.
    \item For $p \geq 2$ and $\lambda < d(1-\tfrac{p}{2}) + \tfrac{p}{2}$ the product $\ast$ cannot be defined (Section \ref{sec: Necconditions}). Here, we will see that the integral kernel of the product \eqref{eq: Algebrenhomomorphismus} depends on an integral over the two kernels of the factors (see \eqref{eq: w3MN}). The condition $\lambda \geq d(1-\tfrac{p}{2}) + \tfrac{p}{2}$ turns out to be necessary for the existence of this integral.
    \item For $p \geq 2$, $\lambda \geq d(1-\tfrac{p}{2}) + \tfrac{p}{2}$ and $\liminf_{M \to \infty} \tfrac{D(M)}{D(M+1)} \geq C_1 > 0$, there is no finite constant $C^\prime_{D, \lambda, p}$ such that \eqref{eq: QuasiSubmultipl} holds (Theorem \ref{thm: keineSubmulti}, Theorem \ref{thm: punendlich}). We construct two elements $\underline{w}(\epsilon), \underline{v}(\epsilon) \in \mathcal{W}^D_{\lambda, p}$ depending on a parameter $\epsilon >0$ such that $\Vert \underline{w}(\epsilon)\Vert^D_{\lambda, p} = \mathrm{const} = \Vert \underline{w}(\epsilon)\Vert^D_{\lambda, p}$ independently of $\epsilon$ and $\lim_{\epsilon \downarrow 0} \Vert (\underline{w}(\epsilon)\ast \underline{v}(\epsilon)) \Vert^D_{\lambda, p} = \infty$. The growth of the combinatorial factors in the normal-ordered product is the reason for the divergence.
    \item For $p \geq 2$ and $\lim_{M \to \infty} \tfrac{D(M)}{D(M+1)} = 0$, there are elements $\underline{w}, \underline{v} \in \mathcal{W}^D_{\lambda, p}$ such that $\underline{w}\ast \underline{v} \notin \mathcal{W}^D_{\lambda, p}$, i.e., for which $\Vert\underline{w}\ast\underline{v}\Vert^D_{\lambda, p}=\infty$ (Theorem \ref{thm: fastgrowing}). The crucial point in the proof is, that the $(M,N)$ component $(\underline{w}\ast \underline{v})_{M,N}$ of the normal-ordered product depends on lower indices of the factors like $w_{M-m, n}$ (see equation \eqref{eq: w3MN}). This has nothing to do with the combinatorial factors!
\end{itemize}
To illustrate, that these results are in fact non-trivial, we analyse some special cases in Section \ref{sec: specialcases}, where a submultiplicity like \eqref{eq: QuasiSubmultipl} holds but not for the entire Banach-space $\mathcal{W}^D_{\lambda, p}$. They also illustrate the two major difficulties in estimating the norm of the normal-ordered product (see Remark \ref{bem: twodifficulties}).  

==> fastgrowing.tex <==
Regarding Lemma \ref{lem: BeispielFakultaet} and the counterexample in Theorem \ref{thm: keineSubmulti} one might think, that choosing fast increasing weight-functions like $D(M) = M!$ would solve the problems. It is possible to show, however, that $\mathcal{W}^D_{\lambda, p}$ is not a closed algebra with respect to $\ast_\rho$, if we choose weight functions, such that $\tfrac{D(M)}{D(M+1)}\leq \tfrac{\mathrm{const}}{M^\delta}$ for $\delta > 0$.

\begin{theorem} \label{thm: fastgrowing}
Let $p\geq 2, \lambda \geq d(1-\tfrac{p}{2}) + \tfrac{p}{2}, \delta >0$ and $\tfrac{D(M)}{D(M+1)}\leq \tfrac{\mathrm{const}}{M^\delta}$. There are elements $\underline{w}, \underline{v} \in \mathcal{W}^D_{\lambda, p}$, such that $(\underline{w}\ast_\rho \underline{v})\notin \mathcal{W}^D_{\lambda, p}$.
\end{theorem}
\begin{bem}
This includes the case  $D(M)=M!$. Therefore by Lemma \ref{lem: BeispielFakultaet} we already know, that we cannot use the exact same counterexample as in Theorem \ref{thm: keineSubmulti}. However, a small modification of our previous counterexample is sufficient for this purpose.
\end{bem}

\begin{proof}
We start with the $p<\infty$ case. For $m,n \in \mathbb{N}$ we define
\begin{equation}
    \Tilde{w}_{m,n}[r; k_1^m; \Tilde{k}_1^n] = \vert k_1^{m}\vert^{\frac{\lambda}{p}} \vert \Tilde{k}_1^{n}\vert^{\frac{\lambda}{p}} \mathbf{1} \left[\Sigma [k_1^m]\leq \tfrac{\rho}{2} \right] \mathbf{1}\left[\Sigma [\Tilde{k}_1^{n}] \leq \tfrac{\rho}{2}\right]
\end{equation}
and note that
\begin{equation}
\begin{split}
    \Vert \Tilde{w}_{m,n} \Vert^\#_{\lambda, p} &= \Vert \Tilde{w}_{m,n} \Vert_{\lambda, p} = \left(\int_{B_1^{m+n}}\limits \dd k_1^{m} \dd\Tilde{k}_1^n \mathbf{1} \left[\Sigma [k_1^{m}]\leq \tfrac{\rho}{2} \right] \mathbf{1}\left[\Sigma [\Tilde{k}_1^{n}] \leq \tfrac{\rho}{2}\right] \right)^{1/p} \\
    &\eqqcolon I(m)\cdot I(n) < \infty.
\end{split}
\end{equation}
Setting $c_m = \left(D(m)I(m)m^{1+\tfrac{\delta}{2}}\right)^{-1}$ and defining
\begin{equation}
    w_{m,n}[r; k_1^m; \Tilde{k}_1^n] \coloneqq v_{m,n}[r; k_1^m; \Tilde{k}_1^n] \coloneqq c_m \cdot c_n\cdot \Tilde{w}_{m,n}[k_1^m; \Tilde{k}_1^n]
\end{equation}
we have $\underline{w} = (w_{m,n})_{m,n \in \mathbb{N}}, \underline{v}= (v_{m,n})_{m,n \in \mathbb{N}} \in \mathcal{W}^D_{\lambda, p}$ since
\begin{equation}
    \Vert \underline{w}\Vert^D_{\lambda, p} = \Vert \underline{v}\Vert^D_{\lambda, p} = \sum_{M=1}^\infty \sum_{N=1}^\infty \frac{1}{M^{1+\tfrac{\delta}{2}}} \frac{1}{N^{1+ \tfrac{\delta}{2}}} < \infty.
\end{equation}
The $(M,N)$-component of the product is given by
\begin{equation}
\begin{split}
    &(\underline{w}\ast_\rho \underline{v})_{M,N}[k_1^M; \Tilde{k}_1^N]\\
    &= \sum_{m=0}^M \sum_{n=0}^N \sum_{q\geq 0} \binom{m+q}{q}\binom{n+q}{q} q! c_{M-m} c_{n+q} c_{m+q} c_{N-n} \vert k_1^{M}\vert^{\frac{\lambda}{p}} \vert \Tilde{k}_1^{N}\vert^{\frac{\lambda}{p}}\\
    &\quad \mathbf{1}\left[\Sigma[k_{m+1}^M] \leq \tfrac{\rho}{2} \right] \mathbf{1}\left[\Sigma[\Tilde{k}_{n+1}^N] \leq \tfrac{\rho}{2} \right]\\
    &\quad \int_{B_1^q} \limits \frac{\dd x_1^{q}}{\vert x_1^{q}\vert} \vert x_1^{q}\vert^{\frac{2\lambda}{p}} \mathbf{1} \left[\Sigma [k_1^m] + \Sigma [\Tilde{k}_1^n] + \Sigma [x_1^q] \leq \rho \right] \mathbf{1}\left[\Sigma [k_1^m] + \Sigma[x_1^q] \leq \tfrac{\rho}{2} \right] \\
    &\quad\quad \mathbf{1}\left[\Sigma[\Tilde{k}_1^n] + \Sigma[x_1^q] \leq \tfrac{\rho}{2}\right]\\
    &= \vert (\underline{w}\ast_\rho \underline{v})_{M,N}[k_1^M; \Tilde{k}_1^N]\vert .
\end{split}
\end{equation}
Summarizing the characteristic functions and considering only the case $m=n=q=1$, we estimate
\begin{equation}
    \begin{split}
        &\vert (\underline{w}\ast_\rho \underline{v})_{M,N}[k_1^M; \Tilde{k}_1^N]\vert \\
        &\geq 4 c_{M-1}c_{N-1}c_2^2 \vert k_1^{M}\vert^{\frac{\lambda}{p}}\vert \Tilde{k}_1^{N}\vert^{\frac{\lambda}{p}} \mathbf{1}\left[\vert k_1\vert \leq \tfrac{\rho}{2} \right] \mathbf{1}\left[\vert \Tilde{k}_1\vert \leq \tfrac{\rho}{2} \right] \mathbf{1}\left[\Sigma[k_{2}^M] \leq \tfrac{\rho}{2} \right] \mathbf{1}\left[\Sigma[\Tilde{k}_{2}^N] \leq \tfrac{\rho}{2} \right]\\
        &\quad \int_{B_1} \limits \dd^dx \vert x\vert^{\frac{2\lambda - p}{p}} \mathbf{1}\left[\vert x\vert \leq \tfrac{\rho}{2} - \max\{\vert k_1\vert, \vert \Tilde{k}_1\vert \} \right].
    \end{split}
\end{equation}
Writing $A(k_1, \Tilde{k_1})$ for the integral in the last line, this yields an estimate for the $\Vert \cdot\Vert^\#_{\lambda, p}$-norm
\begin{equation}
    \begin{split}
        \Vert (\underline{w}\ast_\rho \underline{v})_{M,N}\Vert^\#_{\lambda, p} =& \Vert (\underline{w}\ast_\rho \underline{v})_{M,N}\Vert_{\lambda, p}\\
        \geq& 4 c_{M-1}c_{N-1}c_2^2 \left\{\int_{B_1^{M-1}}\limits \dd k_2^{M} \mathbf{1}\left[\Sigma[k_{2}^M] \leq \tfrac{\rho}{2} \right] \right\}^{1/p} \left\{M\leftrightarrow N \right\}^{1/p} \\
        & \left(\int_{B_1^2}\limits \dd^dk_1 \dd^d\Tilde{k}_1 \mathbf{1}\left[\vert k_1\vert \leq \tfrac{\rho}{2} \right] \mathbf{1}\left[\vert \Tilde{k}_1\vert \leq \tfrac{\rho}{2}\right] \vert A(k_1, \Tilde{k}_1)\vert^p \right)^{1/p}\\
        \geq& \mathrm{const} \cdot c_{M-1}c_{N-1} I(M-1)I(N-1) \\
        =& \frac{\mathrm{const}}{D(M-1)D(N-1)(M-1)^{1+ \frac{\delta}{2}} (N-1)^{1+ \frac{\delta}{2}}}.
    \end{split}
\end{equation}
By our assumption on the weight functions $D(M)$ this implies the divergence of the $\Vert \cdot \Vert^D_{\lambda, p}$-norm since
\begin{equation}
    \begin{split}
        \Vert (\underline{w}\ast_\rho \underline{v})_{M,N}\Vert^D_{\lambda, p} \geq& \mathrm{const} \left(\sum_{M \geq 2} \frac{D(M)}{D(M-1)(M-1)^{1+ \frac{\delta}{2}}} \right)^2\\
        \geq& \mathrm{const} \left(\sum_{M \geq 2} \frac{1}{(M-1)^{1- \frac{\delta}{2}}} \right)^2 = \infty.
    \end{split}
\end{equation}
Next, we consider $p = \infty$. By replacing $\vert k_1^{m}\vert^{\lambda/p}\vert \Tilde{k}_1^{n}\vert^{\lambda/p}$ with $\vert k_1^{m}\vert^\lambda\vert \Tilde{k}_1^{n}\vert^\lambda$ and $c_m$ by $c_m \coloneqq 1/(D(m)m^{1+\frac{\delta}{2}})$ we have
\begin{equation}
    \begin{split}
        \Vert w_{m,n}\Vert_{\lambda, \infty}^\# = \Vert w_{m,n}\Vert_{\lambda, \infty} = \frac{1}{D(m)m^{1+\frac{\delta}{2}}} \frac{1}{D(n)n^{1+\frac{\delta}{2}}}
    \end{split}
\end{equation}
and hence this sum remains finite,
\begin{equation}
    \Vert \underline{w}\Vert^D_{\lambda, \infty} = \Vert \underline{v}\Vert^D_{\lambda, \infty} = \left(\sum_{m \geq 1} \frac{1}{m^{1+\frac{\delta}{2}}} \right)^2 < \infty.
\end{equation}
Similar to $p<\infty$ we estimate the absolute value of the $(M,N)$-component by considering only the $m=n=q=1$ term and get
\begin{equation}
    \begin{split}
        &\frac{\vert (\underline{w}\ast_\rho \underline{v})_{M,N}[k_1^M; \Tilde{k}_1^N]\vert}{\vert k_1^{M}\vert^\lambda\vert \Tilde{k}_1^{N}\vert^\lambda} \\
        &\geq 4 c_{M-1}c_{N-1}c_2^2 \mathbf{1}\left[\vert k_1\vert \leq \tfrac{\rho}{2} \right] \mathbf{1}\left[\vert \Tilde{k}_1\vert \leq \tfrac{\rho}{2} \right] \mathbf{1}\left[\Sigma[k_{2}^M] \leq \tfrac{\rho}{2} \right] \mathbf{1}\left[\Sigma[\Tilde{k}_{2}^N] \leq \tfrac{\rho}{2} \right]\\
        &\quad \int_{B_1} \limits \dd^dx \vert x\vert^{2\lambda - 1} \mathbf{1}\left[\vert x\vert \leq \tfrac{\rho}{2} - \max\{\vert k_1\vert, \vert \Tilde{k}_1\vert \} \right].
    \end{split}
\end{equation}
This function attains its maximum at the origin $k_1 =...=k_m=0=\Tilde{k}_1=...=\Tilde{k}_N$ such that
\begin{equation}
    \begin{split}
        \Vert (\underline{w}\ast_\rho \underline{v})_{M,N} \Vert^\#_{\lambda, \infty} =& \Vert (\underline{w}\ast_\rho \underline{v})_{M,N} \Vert_{\lambda, \infty}\\
        \geq& 4 c_{M-1}c_{N-1}c_2^2 \int_{B_1} \limits \dd^dx \vert x\vert^{2\lambda - 1} \mathbf{1}\left[\vert x\vert \leq \tfrac{\rho}{2} \right].
    \end{split}
\end{equation}
For $\lambda \leq \tfrac{1-d}{2}$ the divergence of the integral is clear whereas for $\lambda > \tfrac{1-d}{2}$ we have
\begin{equation}
    \Vert (\underline{w}\ast_\rho \underline{v})_{M,N} \Vert^\#_{\lambda, \infty} \geq \frac{4O_{d-1} c_{M-1}c_{N-1}c_2^2}{2\lambda + d-1} \left(\frac{\rho}{2} \right)^{2\lambda + d-1}.
\end{equation}
Nevertheless, in this case the divergence follows from
\begin{equation}
    \begin{split}
        \Vert (\underline{w}\ast_\rho \underline{v})_{M,N} \Vert^D_{\lambda, \infty} \geq& \frac{4O_{d-1} c_2^2}{2\lambda + d-1} \left(\frac{\rho}{2} \right)^{2\lambda + d-1} \left(\sum_{M \geq 2} D(M) c_{M-1} \right)^2\\
        \geq& \frac{4O_{d-1} c_2^2}{2\lambda + d-1} \left(\frac{\rho}{2} \right)^{2\lambda + d-1} \left(\sum_{M \geq 2} \frac{\mathrm{const}}{(M-1)^{1- \frac{\delta}{2}}} \right)^2 = \infty.
    \end{split}
\end{equation}
\end{proof}
